Imaging particle collision data for event classification using machine learning

We propose a method to organize experimental data from particle collision experiments in a general format which can enable a simple visualisation and effective classification of collision data using machine learning techniques. The method is based on sparse fixed-size matrices with single- and two-particle variables containing information on identified particles and jets. We illustrate this method using an example of searches for new physics at the LHC experiments.

==> correlations.tex <==
\begin{tabular}{c|c|c}
C &  (r1,c1)  & (r2, c2) \\ \hline  
0.92 &  2,1 & 3,1 \\
0.87 &  5,2 & 5,5 \\
0.87 & 1,1 & 2,1 \\
0.83 &  1,1 & 3,1 \\
0.82 &  3,1 & 4,1 \\
0.81 &  5,2 & 5,3 \\
0.80 &  6,2 & 6,3 \\
0.80 &  6,1 & 6,2 \\
0.79 &  6,2 & 6,5 \\
0.79 &  5,3 & 5,5 \\
0.79 &  4,6 & 6,4 \\
0.79 &  2,2 & 3,2 \\
0.78 &  2,1 & 4,1 \\
0.77 &  2,6 & 6,2 \\
0.76 &  6,1 & 6,5 \\
0.76 &  3,6 & 6,3 \\
0.75 &  5,3 & 5,4 \\
0.74 &  6,3 & 6,5 \\
0.74 &  5,1 & 5,2 \\
0.74 &  4,5 & 5,4 \\
0.74 &  1,1 & 4,1 \\
0.72 &  6,5 & 6,6 \\
0.72 & 5,6 & 6,5 \\
0.71 &  5,2 & 5,4 \\
0.70 &  3,5 & 5,3 \\
0.69 &  5,1 & 5,5 \\
0.69 &  1,6 & 6,1 \\
0.68 &  6,3 & 6,4 \\
0.68 &  6,1 & 6,3 \\
0.67 &  5,4 & 5,5 \\
0.67 &  3,4 & 4,3 \\
0.66 &  6,1 & 6,6 \\
0.65 &  5,1 & 5,3 \\
0.65 &  1,6 & 6,2 \\
0.63 &  6,2 & 6,6 \\
0.63 &  5,6 & 6,2 \\
0.62 &  2,5 & 5,2 \\
0.62 &  1,6 & 2,6 \\
0.61 &  3,6 & 6,4 \\
0.60 &  4,2 & 4,3 \\
0.60 &  3,6 & 4,6 \\
0.59 &  2,6 & 5,6 \\
0.59 &  2,4 & 4,2 \\
0.58 &  6,2 & 6,4 \\
0.58 &  2,2 & 4,2 \\
0.57 &  3,2 & 4,2 \\
0.57 &  2,6 & 6,1 \\
0.55 &  5,6 & 6,3 \\
0.54 &  6,3 & 6,6 \\
0.54 &  5,1 & 5,4 \\
0.54 &  3,6 & 6,2 \\
0.53 & 5,6 & 6,1 \\
0.53 &  1,6 & 6,5 \\
0.53 &  1,6 & 6,3 \\
0.53 &  1,6 & 5,6 \\
0.52 &  1,5 & 2,5 \\
0.51 &  2,6 & 6,5 \\
0.51 &  2,6 & 6,3 \\
0.50 &  6,4 & 6,5 \\
0.49 &  3,6 & 6,5 \\
0.49 &  3,2 & 4,3 \\
0.48 &  4,6 & 6,3 \\
0.47 & 3,6 & 5,6 \\
0.47 &  1,6 & 3,6 \\
0.47 &  1,5 & 3,5 \\
0.46 &  1,5 & 5,3 \\
0.46 &  1,5 & 5,2 \\
0.46 &  1,5 & 5,1 \\
0.45 &  3,6 & 6,1 \\
0.45 &  2,5 & 5,3 \\
0.45 & 2,5 & 3,5 \\
0.45 &  1,5 & 4,5 \\
0.44 &  6,1 & 6,4 \\
0.44 &  3,5 & 5,4 \\
0.44 &  3,5 & 5,2 \\
0.44 &  2,6 & 3,6 \\
0.43 &  5,6 & 6,6 \\
0.43 &  4,5 & 5,3 \\
0.43 &  2,6 & 6,6 \\
0.43 &  1,6 & 6,6 \\
0.43 &  1,5 & 5,4 \\
0.42 & 5,6 & 6,4 \\
0.42 &  3,5 & 4,5 \\
0.42 &  3,2 & 4,4 \\
0.41 &  2,3 & 3,2 \\
0.40 &  2,5 & 5,4 \\
0.40 &  2,5 & 4,5 \\
0.40 &  2,2 & 4,3 \\
0.40 &  1,4 & 2,4 \\
0.39 &  4,5 & 5,2 \\
0.38 &  2,5 & 5,1 \\
0.37 &  1,6 & 6,4 \\
0.37 &  1,6 & 4,6 \\
0.37 &  1,4 & 3,4 \\
0.37 &  1,1 & 5,1 \\
0.36 &  6,4 & 6,6 \\
0.36 &  3,5 & 5,1 \\
0.35 &  3,6 & 6,6 \\
0.34 & 3,5 & 5,5 \\
0.34 &  2,5 & 5,5 \\
0.34 & 2,2 & 4,4 \\
0.34 &  2,1 & 5,1 \\
0.34 &  1,5 & 5,5 \\
0.33 & 4,6 & 6,2 \\
0.33 &  2,4 & 3,4 \\
0.32 &  2,6 & 6,4 \\
0.32 &  1,3 & 2,3 \\
0.30 &  4,5 & 5,1 \\
0.29 &  4,5 & 5,5 \\
0.29 &  3,1 & 5,1 \\
0.29 &  2,1 & 2,2 \\
0.29 &  1,4 & 4,3 \\
0.29 &  1,4 & 4,2 \\
0.28 &  4,6 & 6,1 \\
0.28 &  2,1 & 3,3 \\
0.27 &  4,6 & 6,5 \\
0.27 &  4,6 & 5,6 \\
0.27 &  2,4 & 4,3 \\
0.26 &  4,1 & 4,3 \\
0.26 &  2,3 & 3,4 \\
0.25 &  2,2 & 3,3 \\
0.25 &  1,3 & 3,4 \\
0.25 &  1,2 & 2,3 \\
0.24 &  4,3 & 4,4 \\
0.24 &  4,2 & 4,4 \\
0.24 & 3,4 & 4,2 \\
0.24 &  1,1 & 3,3 \\
0.23 &  4,1 & 5,1 \\
0.23 &  3,3 & 4,4 \\
0.23 &  2,2 & 3,1 \\
0.22 &  5,5 & 6,6 \\
0.22 &  4,1 & 4,2 \\
0.22 &  2,3 & 2,4 \\
0.22 &  1,2 & 2,4 \\
0.21 &  5,5 & 6,5 \\
0.21 &  5,1 & 6,1 \\
0.21 &  4,6 & 6,6 \\
0.21 &  2,1 & 5,2 \\
0.20 &  4,1 & 5,4 \\
0.18 &  5,1 & 6,6 \\
0.18 &  3,1 & 5,3 \\
0.18 &  1,4 & 4,1 \\
0.17 &  5,5 & 6,2 \\
0.17 &  5,5 & 6,1 \\
0.17 &  5,1 & 6,5 \\
0.17 &  5,1 & 6,2 \\
0.17 &  2,6 & 4,6 \\
0.17 &  1,1 & 5,2 \\
0.16 & 3,3 & 4,3 \\
0.16 &  3,1 & 3,3 \\
0.16 & 3,1 & 3,2 \\
0.16 &  2,2 & 4,1 \\
0.16 &  2,1 & 5,3 \\
0.15 &  5,5 & 6,3 \\
0.15 &  5,2 & 6,5 \\
0.15 &  5,2 & 6,2 \\
0.15 &  3,4 & 4,1 \\
0.15 &  3,1 & 5,2 \\
0.15 &  1,4 & 4,4 \\
0.14 &  5,4 & 6,4 \\
0.14 &  5,3 & 6,3 \\
0.14 &  5,3 & 6,2 \\
0.14 & 5,2 & 6,6 \\
0.14 &  5,1 & 6,3 \\
0.14 &  3,3 & 5,2 \\
0.14 &  3,2 & 3,4 \\
0.14 &  3,1 & 5,4 \\
0.14 &  2,3 & 4,3 \\
0.14 &  2,3 & 3,5 \\
0.13 &  5,3 & 6,5 \\
0.13 &  5,2 & 6,3 \\
0.13 &  5,2 & 6,1 \\
0.13 &  4,1 & 5,3 \\
0.13 &  2,4 & 4,5 \\
0.13 &  2,4 & 4,1 \\
0.13 &  2,1 & 5,5 \\
0.13 &  2,1 & 5,4 \\
0.13 &  1,4 & 4,5 \\
0.13 &  1,2 & 2,2 \\
0.13 &  1,1 & 5,3 \\
0.12 &  5,3 & 6,6 \\
0.12 &  4,2 & 5,5 \\
0.12 &  4,2 & 5,1 \\
0.12 &  4,1 & 4,5 \\
0.12 &  3,4 & 4,5 \\
0.12 &  2,4 & 3,2 \\
0.12 &  2,1 & 3,2 \\
0.12 &  1,6 & 5,1 \\
0.12 &  1,1 & 5,5 \\
0.12 &  1,1 & 4,2 \\
0.11 &  5,5 & 5,6 \\
0.11 &  5,4 & 6,5 \\
0.11 &  5,4 & 6,3 \\
0.11 &  5,3 & 6,4 \\
0.11 &  5,3 & 6,1 \\
0.11 &  5,1 & 5,6 \\
0.11 &  4,1 & 5,2 \\
0.11 &  3,3 & 5,1 \\
0.11 &  3,3 & 4,1 \\
-0.11 & 2,2 & 5,5 \\
0.11 &  3,1 & 4,3 \\
0.11 &  2,6 & 5,1 \\
0.11 &  1,6 & 5,5 \\
0.11 &  1,3 & 3,5 \\
0.11 &  1,3 & 1,4 \\
0.11 &  1,1 & 5,4 \\
-0.11 &  1,1 & 4,4 \\
0.10 &  5,5 & 6,4 \\
0.10 &  5,4 & 6,2 \\
0.10 &  5,4 & 5,6 \\
0.10 &  5,2 & 5,6 \\
0.10 &  4,5 & 6,4 \\
0.10 &  4,5 & 5,6 \\
0.10 &  3,1 & 3,5 \\
0.10 &  2,6 & 5,5 \\
0.10 &  2,3 & 4,2 \\
0.10 &  1,3 & 4,3 \\
0.10 &  1,3 & 3,1 \\
-0.10 &  1,1 & 3,2 \\
\end{tabular}

